PhishLang: A Real-Time, Fully Client-Side Phishing Detection Framework Using MobileBERT

In this paper, we introduce PhishLang, the first fully client-side anti-phishing framework built on a lightweight ensemble framework that utilizes advanced language models to analyze the contextual features of a website's source code and URL. Unlike traditional heuristic or machine learning approaches that rely on static features and struggle to adapt to evolving threats, or deep learning models that are computationally intensive, our approach utilizes MobileBERT, a fast and memory-efficient variant of the BERT architecture, to capture nuanced features indicative of phishing attacks. To further enhance detection accuracy, PhishLang employs a multi-modal ensemble approach, combining both the URL and Source detection models. This architecture ensures robustness by allowing one model to compensate for scenarios where the other may fail, or if both models provide ambiguous inferences. As a result, PhishLang excels at detecting both regular and evasive phishing threats, including zero-day attacks, outperforming popular anti-phishing tools, while operating without relying on external blocklists and safeguarding user privacy by ensuring that browser history remains entirely local and unshared. We release PhishLang as a Chromium browser extension and also open-source the framework to aid the research community.

==> tables/browser.tex <==
\begin{table*}[]
\begin{tabular}{|c|c|ccc|ccc|ccc|}
\hline
\multirow{2}{*}{Attack Type} & \multirow{2}{*}{\# URL} & \multicolumn{3}{c|}{Safe Browsing}                                        & \multicolumn{3}{c|}{SmartScreen}                                          & \multicolumn{3}{c|}{SiteCheck}                                            \\ \cline{3-11} 
                             &                         & \multicolumn{1}{c|}{Initial} & \multicolumn{1}{c|}{Subsequent} & Time     & \multicolumn{1}{c|}{Initial} & \multicolumn{1}{c|}{Subsequent} & Time     & \multicolumn{1}{c|}{Initial} & \multicolumn{1}{c|}{Subsequent} & Time     \\ \hline
Regular Attack               & 1,595                   & \multicolumn{1}{c|}{50.92}   & \multicolumn{1}{c|}{84.33}      & 3.71 hrs & \multicolumn{1}{c|}{34.26}   & \multicolumn{1}{c|}{74.26}      & 5.85 hrs & \multicolumn{1}{c|}{17.46}   & \multicolumn{1}{c|}{76.37}      & 3.53 hrs \\ \hline
JS Evasion                   & 306                     & \multicolumn{1}{c|}{35.27}   & \multicolumn{1}{c|}{70.36}      & 5.67 hrs & \multicolumn{1}{c|}{27.48}   & \multicolumn{1}{c|}{75.42}      & 9.66 hrs & \multicolumn{1}{c|}{30.13}   & \multicolumn{1}{c|}{71.62}      & 3.18 hrs \\ \hline
ReCAPTCHA/QR                 & 91                      & \multicolumn{1}{c|}{40.97}   & \multicolumn{1}{c|}{66.07}      & 3.75 hrs & \multicolumn{1}{c|}{15.31}   & \multicolumn{1}{c|}{81.34}      & 7.54 hrs & \multicolumn{1}{c|}{11.2}    & \multicolumn{1}{c|}{58.09}      & 2.05 hrs \\ \hline
Clickjacking                 & 325                     & \multicolumn{1}{c|}{61.32}   & \multicolumn{1}{c|}{80.28}      & 2.42 hrs & \multicolumn{1}{c|}{38.48}   & \multicolumn{1}{c|}{77.65}      & 5.3 hrs  & \multicolumn{1}{c|}{26.31}   & \multicolumn{1}{c|}{78.22}      & 4.37 hrs \\ \hline
DOM Attacks                  & 102                     & \multicolumn{1}{c|}{55.79}   & \multicolumn{1}{c|}{74.39}      & 3.48 hrs & \multicolumn{1}{c|}{18.27}   & \multicolumn{1}{c|}{85.36}      & 5.56 hrs & \multicolumn{1}{c|}{8.27}    & \multicolumn{1}{c|}{81.2}       & 3.06 hrs \\ \hline
Text encoding                & 81                      & \multicolumn{1}{c|}{27.97}   & \multicolumn{1}{c|}{72.57}      & 6.45 hrs & \multicolumn{1}{c|}{20.79}   & \multicolumn{1}{c|}{70.6}       & 2.5 hrs  & \multicolumn{1}{c|}{15.5}    & \multicolumn{1}{c|}{89.14}      & 1.24 hrs \\ \hline
\end{tabular}
\end{table*}


==> text/detection.tex <==
\subsection{Common phrases in model detection}
\label{common_phrases_in_phishing}
\label{prompt_detection_ml}

\begin{table}[htbp]
\centering
\renewcommand{\arraystretch}{1.2}
\caption{Distribution of common phishing phrases and confidence scores}
\begin{tabular}{p{4cm}|c|c}
\hline
\multicolumn{1}{c|}{Phrase} & \multicolumn{1}{c|}{Appearance} & \multicolumn{1}{c}{Median Confidence} \\
\hline\hline
Verify your account info. & 13.71\% & 0.972 \\
Click to reset password & 10.23\% & 0.951 \\
Account suspension warning & 8.25\% & 0.782 \\
View your bill & 6.63\% & 0.941 \\
Order shipped notification & 6.14\% & 0.896 \\
Billing error, update info & 3.62\% & 0.805 \\
Track your package & 3.69\% & 0.853 \\
Prescription ready & 2.87\% & 0.928 \\
Account on hold & 2.78\% & 0.689 \\
Verify account, please & 2.51\% & 0.826 \\
Review login attempts & 2.08\% & 0.884 \\
Subscription expiring & 1.75\% & 0.698 \\
Confirm mailing address & 1.51\% & 0.839 \\
Payment processing issue & 1.14\% & 0.762 \\
Review recent transactions & 0.88\% & 0.813 \\
Unauthorized login attempt & 1.87\% & 0.964 \\
Compromised account & 0.78\% & 0.755 \\
Verify your identity & 0.70\% & 0.861 \\
Update credit card details & 0.50\% & 0.783 \\
New message waiting & 0.46\% & 0.801 \\
\hline
\end{tabular}
\label{common_phrases}
\end{table}

During our model prediction stage, we identified how it focuses on several deceptive phrases used in the scam resources and how it contributes towards a positive prediction label (i.e. Phishing). The prevalence and confidence scores associated with these phrases offer insightful trends. For example, 
"Verify your account information" emerged as the most prevalent phrase, found in approximately 13.71\% of the sites. This dominance suggests a favored tactic by scammers, leveraging the importance of account security. The high confidence score of 0.972 underscores the model's ability to detect such prominent schemes. Urgency and intimidation tactics are notable across several phrases. For instance, terms hinting at account suspension, potential billing errors, or compromised security details reflect scammers' efforts to instill fear and prompt hurried reactions. This sense of urgency, combined with seemingly routine notifications like bill availability or shipped orders, showcases the duality of the phishing landscape. 

Interestingly, while phrases related to daily activities such as shipping notifications or prescription readiness were less frequent, their confidence scores remained consistently high. This suggests that irrespective of their frequency, the model is adept at pinpointing this potentially deceptive intent. Conversely, certain phrases like "Update your credit card details" or "New message waiting" were less prevalent, yet they still attracted substantial confidence scores. This highlights that the model is also capable of detecting less common strategies.

In summary, our analysis provides a quantitative look into the different strategies or intentions used by scammers to entice users into sharing their sensitive data, as well as how our model performs at identifying them. 

\subsection{Detecting evasive phishing threats}

Prior literature has highlighted how regular phishing detection entities struggle to identify evasive phishing attacks (such as client/server-side evasions~\cite{oest2020phishtime}). However, most of these detection measures are reliant on URL, DOM, or HTML-based features which are easier to manipulate than the actual appearance of the website. This is because the later needs to have a deterministic layout to appear "convincing" to the potential victim. For example, a Chase bank phishing page would almost always contain credential fields, and some form of lure to entice the victim into sharing their information. In fact, more recent models that infer phishing intention from the appearance of the websites~\cite{lin2021phishpedia,liu2022inferring,afroz2011phishzoo} have been found to be fairly effective against several evasive threats. However, these models rely on image screenshots of the website, processing which is a very time and resource-consuming activity that can significantly slow down the detection and reporting of new threats. Thus, using several heuristics that have been highlighted for these attacks~\cite{liang2016cracking,browserinbrowser:2022,oest2019phishfarm,han2016phisheye} we pinpoint the detection efficiency of ScamLLM against these attacks. Overall, we identified 1,971 URLs that hosted seven distinct evasive attacks in our test set. Table~\ref{table:summary_phishing_attacks} contains descriptions of the different evasive attacks, and Table~\ref{table:performance_evasive_attacks} shows the performance of ScamLLM against these threats. 

\begin{table*}[h]
\centering
\caption{Summary of Phishing Attack Types}
\label{table:summary_phishing_attacks}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cp{0.25\textwidth}p{0.75\textwidth}}
\hline
\textbf{Attack No.} & \textbf{Attack Type} & \textbf{Attack Description} \\
\hline
1 & ReCAPTCHA attacks & An attack that presents a fake login page with a reCAPTCHA challenge to capture credentials~\cite{kang2009captcha,kang2010captcha,unit42-captcha-phishing,trustwave-phishing-captcha,odeh2021machine,google-recaptcha-display}. \\
\hline
2 & QR Code attacks & An attacker shares a website containing a QR code that leads to a phishing website~\cite{securitymagazine-qr-phishing,pcmag-qr-phishing-fbi,vidas2013qrishing,qrserver}. \\
\hline
% 4 & Phishing button attacks & Attacks that use a fake webpage with a button that redirects the user to a phishing website. \\
% \hline
3 & Browser-in-the-Browser attacks & A deceptive pop-up mimics a web browser inside the actual browser to obtain sensitive user data~\cite{mrd0x-phishing}. \\
\hline
4 & iFrame injection/Clickjacking & Attackers use iFrames to load a malicious website inside a legitimate one~\cite{secnhack-iframe-injection,auth0-clickjacking,portswigger-same-origin-policy}. \\
\hline
5 & Exploiting DOM classifiers & Phishing websites designed to avoid detection by specific anti-phishing classifiers~\cite{liang2016cracking}. \\
\hline
6 & Polymorphic URL & Attacks that generate a new URL each time the website is accessed~\cite{cofense-phishing-attack,lam2009counteracting}. \\
\hline
7 & Text encoding exploit & Text in the credential fields is encoded such that it is not recognizable from the website's source code~\cite{cybersecurityventures_punycode_phishing,fouss2019punyvis}. \\
\hline
% 10 & Browser fingerprinting attacks & Phishing pages are only rendered when visited through specific agents~\cite{laperdrix2020browser,upathilake2015classification,safebrowsing}. \\
% \hline
\end{tabular}
}
\end{table*}

\begin{table*}[h]
\centering
\caption{Performance of ScamLLM against evasive phishing attacks}
\label{table:performance_evasive_attacks}
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{cccccc}
\hline
\textbf{Attack No.} & \textbf{Attack Type} & \textbf{Samples} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} \\
\hline
1 & ReCAPTCHA attacks & 350 & 92.5\% & 90.1\% & 88.3\% \\
\hline
2 & QR Code attacks & 225 & 94.2\% & 95.3\% & 93.7\% \\
\hline
3 & Browser-in-the-Browser attacks & 412 & 89.8\% & 88.6\% & 87.9\% \\
\hline
4 & iFrame injection/Clickjacking & 167 & 91.3\% & 92.1\% & 90.5\% \\
\hline
5 & Exploiting DOM classifiers & 287 & 88.4\% & 89.0\% & 85.1\% \\
\hline
6 & Polymorphic URL & 259 & 95.1\% & 93.8\% & 94.4\% \\
\hline
7 & Text encoding exploit & 271 & 90.7\% & 91.2\% & 89.9\% \\
\hline
\end{tabular}}

\end{table*}

\section{Brand and event detection}

\subsection{Keyword based matching}
Detecting the brand and organization targeted by the scam is crucial information for the prompt takedown of the attacks by notifying the concerned parties~\cite{oest2020phishtime}. Prior work has identified brand logos by using image recognition models~\cite{lin2021phishpedia,afroz2011phishzoo} which are not only computationally expensive, but attackers can easily evade them by modifying pixel level density of the images or using alternate/new logos which these logo detection models might not have been trained on. In contrast, we extract the brand from the text of the scam and consequently identify the event of the scam based on the brand that is being targeted. We utilize 392 unique brands identified by OpenPhish~\cite{openphish_brands} that are targetted by scams. These brands are spread across 17 categories such as financial institutions, telecommunications, logistics \& couriers, e-commerce, transportation, online/cloud services, cryptocurrency, payment services, social networking platforms, gaming, insurance, gambling etc. We utilize NLTK's Named entity recognition library to identify the phrase/keyword in the scam that mentions an organization. We then utilize the Levenshtein distance algorithm (\emph{t>0.8)} to match the phrase with an organization in our list. In scams where a brand phrase is not found, we use the same distance-matching approach to match the URL attached in the scam message with the domains of the known organizations in our list. Finally, after an organization is matched, we assign one of the 17 categories (events). 




\section{Email and regular scam detection}

\subsection{Transferability and finetuning of detection models}
To detect email-based scams, we first evaluated our DeBERTA model trained using the phishing dataset on the set of 17,041 phishing emails (from APWG) and the same number of benign emails from the Enron email dataset. We found that this model had a precision of 71\%, with true positive detections focusing primarily on the list of keywords common to phishing attacks found in Section~\ref{common_phrases_in_phishing}, and false negatives being prone to emails that did not have a credential-taking intention, but attempted to engage the user in a way that would lead to a social engineering effort in the future (Such as providing technical support for an "infected" system). We saw a similar pattern for SMS-based scams, where the model had a precision of 76\%.
On the other hand, our brand detection model had a similar performance at detecting the organization targeted by both email and SMS-based scams, with a precision of 97\% for emails, and 94\% for SMS. 
Thus, we decided to fine-tune our phishing detection model to improve its capabilities for detecting email and SMS-based scams.
We decided to fine-tune, instead of re-training the DeBERTA model from scratch, since both email and SMS scams evidently share characteristics with phishing websites, but can be further improved by being able to recognize the nuances that these scams contain. 
We fine-tuned our classifier for email-based detection by using 17,041 malicious emails, and 17,041 benign emails. Similarly, we did the same with 4,079 malicious SMS and the same number of benign SMS. The fine-tuning improved the precision of detection of email scams to 96\% and the precision for detecting SMS-based scams to 94\%. The detailed performance metrics for the models are illustrated in Table~\ref{tab:email_sms_model_performance}.

\begin{table*}[h]
\centering
\caption{Model Performance on Email and SMS Scams}
\label{tab:email_sms_model_performance}
\begin{tabular}{|l|c|c|c|c|c|c|}

\hline
Model            & \multicolumn{3}{c|}{Email scam}                & \multicolumn{3}{c|}{SMS scam}                  \\ \hline
                 & Accuracy       & Precision      & Recall      & Accuracy       & Precision      & Recall      \\ \hline
DistilBERT-base  & 0.43           & 0.50           & 0.45        & 0.37           & 0.45           & 0.40        \\ \hline
DistilBERT-phish & 0.60           & 0.71           & 0.65        & 0.65           & 0.76           & 0.70        \\ \hline
DistilBERT-finetuned  & 0.90           & 0.96           & 0.92        & 0.88           & 0.94           & 0.90        \\ \hline
\end{tabular}

\end{table*}


\begin{table}[h]
\centering
\resizebox{1\columnwidth}{!}{%
\caption{Model Performance on Email and SMS Scams}
\label{tab:model_performance}
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
Model            & \multicolumn{3}{c|}{Email scam}                & \multicolumn{3}{c|}{SMS scam}                  \\ \hline
                 & Accuracy       & Precision      & Recall      & Accuracy       & Precision      & Recall      \\ \hline
DistilBERT-base  & 0.43           & 0.50           & 0.45        & 0.37           & 0.45           & 0.40        \\ \hline
DistilBERT-phish & 0.60           & 0.71           & 0.65        & 0.65           & 0.76           & 0.70        \\ \hline
DistilBERT-finetuned  & 0.90           & 0.96           & 0.92        & 0.88           & 0.94           & 0.90        \\ \hline
\end{tabular}}

\end{table}

\section{Application of ScamLLM}

\subsection{Comparison with anti-phishing measures}

A common practice to evaluate the effectiveness of new phishing detection models is to compare their performance with popular and established anti-phishing blocklists and tools~\cite{oest2020phishtime,oest2020sunrise}. 
Thus, to further identify the effectiveness of our model, we check how well phishing URLs that were identified by ScamLLM were detected by popular blocklists: Google Safe Browsing (GSB)~\cite{safebrowsing}, PhishTank~\cite{phishtank}, OpenPhish~\cite{openphish} and APWG eCrimeX~\cite{ecrimex:2022}. 
GSB is regularly used on several browsers running on the Chromium engine, such as Google Chrome ~\cite{chromesafebrowsing}, Firefox ~\cite{firefox:2021}, Vivaldi~\cite{vivaldisafebrowsing}, etc., while PhishTank and OpenPhish regularly contribute their data to several anti-phishing tools and web browsers ~\cite{phishfriends}. 
APWG's eCrimeX also shares its data with several organizational anti-phishing entities~\cite{oest2020phishtime}. We also checked the URLs with 80 different antiphishing tools using VirusTotal. To identify new phishing URLs, we run ScamLLM over Certstream~\cite{certstream:2022}. Certstream is a Certificate Transparency log database that notes all domains that obtain SSL certification and is a popular resource for identifying new online scams. We ran our analysis for 32 days, from September 28th, 2023 to October 30th, 2023, identifying 8,314 new phishing URLs. We further identified how many of these URLs were regular phishing attacks (n=6,045) i.e. having credential fields and organization logo, and how many were evasive (n=2,269), such as those underlined in Table~\ref{table:performance_evasive_attacks}. For our analysis, we look at the two main aspects of URL blocklisting, \textit{Coverage} -  that denotes what percentage of the URLs were identified as phishing by the respective blocklist during our analysis, and \textit{Response time} - how quickly the URL was detected by a blocklist after being identified by ScamLLM. 

\subsubsection{}{Anti-phishing blocklists:}
For each phishing URL identified by ScamLLM, we checked if it was present on any of the blocklists at regular intervals of 10 minutes till the URL became inactive. Out of 8,314 URLs identified by ScamLLM, 792 were already detected by one or more blocklists. So we do not include them in the analysis for the respective blocklists (that detected them).  
Table~\ref{table-fhd-overall} provides a comparative analysis of the efficacy of PhishTank, OpenPhish, Google Safe Browsing (GSB), and eCrimeX in mitigating regular and evasive phishing attacks which were found by ScamLLM.
GSB shows very good coverage of 91.0\% for regular phishing attacks with a median response time of just 30 minutes. 
PhishTank, although less effective than GSB, shows coverage of 47.5\% for regular phishing attacks with a median response time of 1 hour and 45 minutes, 
On the other hand, OpenPhish and eCrimeX stand at 59.2\% and 75.6\% coverage against regular phishing threats respectively, demonstrating a quick median response time of about an hour.
However, the blocklists struggled against evasive phishing threats. For example, Google Safe Browsing's performance fell to 57.3\% coverage with a 2 hours and 10 minutes median response time against evasive phishing attacks, whereas PhishTank's coverage dropped to 14.8\%, and the median response time slowed down to 3 hours and 50 minutes.
Again OpenPhish and eCrimex had their coverage diminished to 22.6\% and the median response time lags to 4 hours and 30 minutes and 35\% with a response time extended significantly to 5 hours, respectively.
Prior literature has explored how anti-phishing blocklists often struggle against such evasive threats, especially those that utilize adversarial means in the form of domain, website source(or DOM), or credential field manipulation~\cite{liang2016cracking}. With a significant gap in both coverage and response time between ScamLLM and these blocklists, ScamLLM can prove useful in contributing newer phishing URLs to blocklists.

\begin{table*}[]
\centering
\caption{Blocklisting performance and response time of anti-phishing entities against phishing attacks.}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{|c|ccc|ccc|}
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{Regular Phishing Attacks}} & \multicolumn{3}{c|}{\textbf{Evasive Phishing Attacks}} \\ \cline{2-7} 
 & \multicolumn{1}{c|}{\textbf{Coverage}} & \multicolumn{1}{c|}{\textbf{Min/Max (hh:mm)}} & \textbf{Median Speed (hh:mm)} & \multicolumn{1}{c|}{\textbf{Coverage}} & \multicolumn{1}{c|}{\textbf{Min/Max (hh:mm)}} & \textbf{Median Speed (hh:mm)} \\ \hline
PhishTank & \multicolumn{1}{c|}{47.5\%} & \multicolumn{1}{c|}{0:02/48:30} & 01:45 & \multicolumn{1}{c|}{14.8\%} & \multicolumn{1}{c|}{0:10/96:20} & 03:50 \\ 
OpenPhish & \multicolumn{1}{c|}{59.2\%} & \multicolumn{1}{c|}{0:01/36:45} & 00:58 & \multicolumn{1}{c|}{22.6\%} & \multicolumn{1}{c|}{0:15/120:00} & 04:30 \\ 
GSB & \multicolumn{1}{c|}{91.0\%} & \multicolumn{1}{c|}{0:00/24:00} & 00:30 & \multicolumn{1}{c|}{57.3\%} & \multicolumn{1}{c|}{0:08/80:40} & 02:10 \\ 
eCrimeX & \multicolumn{1}{c|}{75.6\%} & \multicolumn{1}{c|}{0:03/30:00} & 01:20 & \multicolumn{1}{c|}{35.0\%} & \multicolumn{1}{c|}{0:20/110:50} & 05:00 \\ 
Hosting Domain & \multicolumn{1}{c|}{82.7\%} & \multicolumn{1}{c|}{0:02/33:30} & 01:10 & \multicolumn{1}{c|}{60.2\%} & \multicolumn{1}{c|}{0:25/150:00} & 03:30 \\ \hline

\hline
\end{tabular}}
\label{table-fhd-overall}
\end{table*}


\subsubsection{Anti-phishing tool analysis:} We also used VirusTotal~\cite{virustotal} to scan URLs detected as phishing by ScamLLM at intervals of every 10 mins, from when the URL first appeared in our dataset, up till when it became inactive, or up to a week, whichever was sooner. 
This is to mitigate the possibility of outdated scores~\cite{vtpaper_blackbox}. 
Unlike our previous analysis, where we evaluated the performance of each blocklist separately, we aggregated the VirusTotal scores, which provided the detection rate for 80 different anti-phishing engines and blocklists. VirusTotal data also includes GSB, PhishTank, and OpenPhish, and we excluded the scores of these blocklists to avoid redundancy with our previous analysis. Figure~\ref{fig:tool_detection} shows the cumulative distribution of detection rates for both regular and evasive phishing attacks by these antiphishing tools (truncated up to 20 detections). We find that 50\% of regular phishing URLs had a detection rate of 16 or lower, whereas the same was only 5 detections for evasive phishing URLs. In fact, only 403 evasive URLs had 10 or more detections, whereas 5,059 regular phishing URLs had 10 or more detections. Thus, similar to our blocklisting analysis, we also find that ScamLLM can improve the detection of new phishing URLs, especially those that are evasive in nature. 

\begin{figure}[t]

\centerline{\includegraphics[width=0.8\columnwidth]{figures/detection_rate.pdf}}
\caption{Cumulative distribution of antiphishing detections for regular versus evasive attacks}
\label{fig:tool_detection}
\end{figure}


\subsection{Evaluating misdetections}
\begin{figure*}[t]

\centerline{\includegraphics[width=1.4\columnwidth]{figures/false_postives.pdf}}
\caption{Examples of misdetections (false positives)}
\label{fig:misdetections}
\end{figure*}

To test the robustness of the model, we randomly evaluated 500 websites which were marked as phishing to identify misclassifications. The misclassifications can be primarily divided into two categories:

\subsubsection{Appearence heuristics}Figure~\ref{fig:misdetections} illustrates three explanations that contain the primary characteristics that were mislabeled. Subfigure A contains a QR code along with a download link that leads to an external domain. Since QR codes contain seemingly obfuscated text content (for example a URL) as well as linking to an external domain, it was flagged as phishing by ScamLLM. On the other hand, Subfigure B contains a local web-mail login which was flagged as phishing due to containing a relatively new subdomain, a simplified design, and sensitive credential fields. Finally, Subfigure C contains a Software-as-a-Service brand that is detected due to utilizing the Microsoft logo as well as logos of several payment options (such as Mastercard and Paypal). 
\subsubsection{Inactivity} 
We found nearly 278 samples that were either inactive or parked domains but were marked as Phishing by ScamLLM. Our training ground truth did not contain any inactive samples, which might have led to the classifier defaulting to the Phishing label for this sample (since inactive URLs have very little text on the page, which is in stark contrast to well-designed benign pages). We thus added 25.7k more samples which were inactive pages and 11.4k which were parked (collected from Tranco's list) and added two new labels to the classifier, Inactive and parked. We have a specific label for parked domains since parked domains can be reused to host phishing websites at a later date~\cite{alrwais2014understanding}. Our retrained classifier had an accuracy of 97.08\% on the 30\% split testing set for inactive (n=7,533) and 93.11\% on the 30\% split for parked domains (n=3,489).

\subsection{Malicious email detection}
While the creation of new websites, whether malicious or benign can be monitored using Certstream, no such facility is available for finding new emails and SMS messages.
Ideally, we can set up honeypot accounts (email addresses and SMS phone numbers) that can act as decoy systems to attract and catch cyber attackers. However, doing so would require IRB (Institutional Review Board) approval to carry out the study ethically, since setting up honeypot accounts to attract and monitor cyber attackers brings a likelihood of collecting data that could be linked back to individuals, whether they are the attackers themselves or incidental contacts. We are currently planning to get such approval. Thus, presently, for the initial testing of email-based detection, we monitored the APWG email report list from October 4th to November 22nd, where 5,172 emails were reported, out of which 4,670 emails were detected as malicious by ScamLLM. Considering that the large majority of APWG-reported emails are malicious, our model achieved an accuracy of 90.2\%. It is worth noting that ScamLLM was able to detect both regular credential phishing emails, as well as brand brand-agnostic scam emails. For example, Figure~\ref{fig:email_detection1} shows an example of a credential phishing email purporting to be from Amazon, indicating that the recipient's membership has lapsed and offering an enticing opportunity to renew along with the promise of additional benefits and a gift card.
On the other hand, Figure~\ref{fig:email_detection2} shows an example of a brand-agnostic email scam, where the sender makes an implausible claim about receiving a large compensation payment and instructs the recipient to stop contacting others and instead provide personal details to a supposed representative of an international monetary fund. Figure~\ref{fig:email_events} provides the distribution for the events that were targeted by the email scams identified by ScamLLM. 

\begin{figure}[t]
    \centering
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=1\columnwidth]{figures/credential_phish_example.pdf}
        \caption{Detecting a credential phishing email}
        \label{fig:email_detection1}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=1\columnwidth]{figures/non_credential_email_example.pdf}
        \caption{Detecting a brand-agnostic email scam }
        \label{fig:email_detection2}
    \end{subfigure}
    \caption{Examples of email scam samples detected by ScamLLM}
    \label{fig:email_detection}
\end{figure}

\begin{figure}[t]

\centerline{\includegraphics[width=0.9\columnwidth]{figures/distribution_of_malicious_emails.pdf}}
\caption{Distrubution of events targeted by email scams}
\label{fig:email_events}
\end{figure}

\section{The ScamLLM Browser extension}

We realize the ScamLLM framework is a browser extension that can be installed on any Chromium based web-browser to protect against phishing and email threats. Unlike other anti-scam/anti-phishing browser extensions~\cite{bitdefender,mcafeewebadvisor}, ScamLLM does not rely on remote blocklists (i.e. a list of known phishing URLs) for detection, and instead, the classification is done entirely by the local LLM model. Figure~\ref{fig:scamllm_extension} shows an example of ScamLLM preventing the user from accessing a suspicious phishing website.
Our goal of building a lightweight browser extension is also justified since ScamLLM has an average footprint of only 72 Megabytes of RAM across all open browser tabs, which is significantly lower than other online protection extensions such as Google Safe Browsing (224 Megabytes on average). Additionally, due to the local classification approach, ScamLLM does not send any URLs or web resources visited by the user to remote servers, thus enforcing user privacy restrictions. It is also the first browser extension that can block email-based scams across any email provider since it does not have to keep track of complex anti-spam rules~\cite{mendez2006comparative}. To prevent SMS-based scams, we plan to extend ScamLLM as an Android application in the near future. 


\begin{figure}[!htb]

\centerline{\includegraphics[width=0.8\columnwidth]{figures/scamllm_running.pdf}}
\caption{Example of ScamLLM blocking a phishing website. Note that the website URL is not redacted since it is already inactive.}
\label{fig:scamllm_extension}
\end{figure}

\section{Discussion and Conclusion}

In this work, we proposed the first anti-scam detection framework based on a large language model. ScamLLM determines the malicious behavior of an online resource by looking only at the text-based content. Firstly, we contribute a data parser that can build a semantic representation of online resources which makes it convenient for the language model to understand the inter-relationship between the objects in the resource and the overall context of the potential scam. By utilizing this parsing approach, our language model was trained on more than 52k malicious and benign online resources, ScamLLM can identify both regular and evasive scams. For example, we find that ScamLLM performs well against several website-based evasive attacks such as QR Code/CAPTCHA attacks, Text encoding, and iFrame injection attacks, which are usually missed by traditional antiphishing vendors. We also found that phishing URLs (including evasive attacks) identified by ScamLLM are often missed by popular anti-phishing blocklists and, thus signifying the impact of running our framework and reporting new attacks to anti-phishing entities and hosting providers. 

We also focus on detecting the organizations and events that are targeted by these scams. Prevalent anti-phishing vendors can only identify a limited set of organizations and are not able to identify the context of the scams at all~\cite{liu2022inferring}. We train ScamLLM such that it can not only identify popular organizations but also identify the intention of the scam. This can lead to the reporting of new organizations that are being targeted, as well as brand-agnostic scams.

Our model finetuned on emails and SMS also shows a similar trend of identifying both branded and brand-agnostic scams. These scams, despite sharing some similarities with phishing websites are significantly different and thus cannot be detected easily by antiphishing vendors~\cite{oest2020sunrise}. Moreover, due to the reliance on text content only, ScamLLM does not need to utilize any anti-spam rules that are usually maintained by email or mobile network providers. However, our evaluation of the email model is limited at this stage of the work. Due to the ethical implications of creating honeypots to track and block incoming scam messages, we are currently planning to get approval from the Institutional Review Board (IRB). Ideally, we plan to have several dummy emails and phone numbers, which would be used to sign up for several mailing lists, surveys, free product trials, etc. Considering that websites often share user data with third-party providers~\cite{mayer2012third}, preparing scam honeypots in this way is commonly done in research. This would also allow us to compare the performance of ScamLLM against the built-in anti-scam protection measures used in popular email services such as Gmail and Outlook. Presently, by testing our model against phishing emails reported by users (via APWG), we found that ScamLLM has a real-life accuracy of nearly 91\%, which is significantly higher than prevalent anti-scam efforts~\cite{oest2020sunrise}. 

Finally, we implement the ScamLLM framework as a Chorimum-based browsing extension. The extension is lightweight, does not rely on any remote blocklist, does not send any user data to the cloud, and for email scams can work across any email provider. The extension provides an accessible way for end-users to protect them for online scams. 

==> text/ethics.tex <==
\section*{Ethical Considerations}

As per the USENIX Security guidelines for ethical considerations, we have included this ethics report in accordance with the principles outlined in their call for papers and submission policies. Our research on phishing website detection through the development and deployment of PhishLang was conducted with a comprehensive review of ethical implications. Our goal was to prioritize user privacy, transparency, and the broader impact on cybersecurity while ensuring the respect and autonomy of individuals, even those engaged in malicious activities.

\subsection*{Stakeholder Considerations}

Key stakeholders in this research include website users, administrators of legitimate and phishing websites, cybersecurity professionals, and the general public. We took special care to ensure no personally identifiable information (PII) was collected or compromised during the study. The PhishLang model was trained on a publicly available dataset (PhishPedia) and its inference (through the real-time framework as well as the browser extension) operates exclusively on metadata accessible from public websites, ensuring no interaction with sensitive or private information. Moreover, our client-side application does not, by default, send any information to external servers, and is fully functional using the user's system resources. 

\subsection*{Consequentialist Ethics}

In alignment with the \textit{Beneficence} principle outlined in The Menlo Report~\cite{bailey2012menlo}, we sought to minimize harm while maximizing the societal benefits of our research. The main long-term benefit is improving phishing detection and enhancing user security through the release of PhishLang, an efficient, accessible and explainable client-side tool. However, we recognize that by publicly disclosing our detection methods, there is a potential risk of malicious actors evolving their tactics to evade detection. However, our adversarial studies (and subsequent patches) are designed such that attempting to evade them would most likely lead to a non-functional website. Moreover, our model is reliant on semantic text analysis of source code, an approach which is not popularly used in other anti-phishing measures, and thus exploiting our model does not indicate compromise of (most) other detection tools.  


\subsection*{Deontological Ethics}

In accordance with the \textit{Respect for Persons} principle, we ensured that no private or personally identifiable information (PII) was accessed, processed, or disclosed. Our team did not interact directly with any phishing website operators or users, focusing solely on publicly available website data and metadata. Since our research did not involve interaction with human subjects or sensitive personal data, it was deemed not to require Institutional Review Board (IRB) approval. It is also worth noting that we do not opensource any data, as our focus is on realising a detection tool. 


\subsection*{Disclosure and Vulnerability Reporting}

When phishing websites were identified using PhishLang, we adhered to responsible disclosure protocols. These websites were promptly (within 3 hours) reported to relevant stakeholders, including affected organizations and platforms (e.g., web hosting providers). In fact our disclosure led to the removal of several evasive threats which were not detected otherwise. Also, all our results in the paper contain only aggregated statistics, ensuring that no specific individuals were identifiable from the results.

\subsection*{Legal and Ethical Compliance}

We ensured that our research complied with all applicable laws and respected the terms of service of platforms we interacted with, particularly the usage of the open-source anti-phishing blocklists and software libraries. No live experiments were conducted that could harm legitimate users or violate platform policies.

\subsection*{Proactive Ethics Consideration}

Ethical considerations were proactively integrated into every stage of the research process, from data collection to the final publication of results. Our decisions were guided by a commitment to minimize harm, enhance transparency, and ensure the broader benefit of the research, with constant evaluation of the potential ethical challenges throughout the study.

\subsection*{Open Science Policy}

In alignment with the Open Science Policy, we have made the PhishLang framework (including scripts to train the model) and the client-side browser extension publicly available. However, due to the sensitive nature of phishing websites, particularly live webpages, we do not release the phishing websites identified by PhishLang publicly. Access to the data can be granted upon request, subject to a legal data-sharing agreement with our organization. While the functionality of our framework and extension can be replicated, a large portion of our analysis relies on real-time data, such as blocklist measurements. Although it is possible to replicate this to some degree, full reproducibility can be challenging.

